Projection of Functionals and Fast Pricing of Exotic Options

We investigate the approximation of path functionals. In particular, we advocate the use of the Karhunen-Lo\`eve expansion, the continuous analogue of Principal Component Analysis, to extract relevant information from the image of a functional. Having accurate estimate of functionals is of paramount importance in the context of exotic derivatives pricing, as presented in the practical applications. Specifically, we show how a simulation-based procedure, which we call the Karhunen-Lo\`eve Monte Carlo (KLMC) algorithm, allows fast and efficient computation of the price of path-dependent options. We also explore the path signature as an alternative tool to project both paths and functionals.

==> Path_Approx/ItoChaos.tex <==
\subsection{Connection with the Wiener-Itô Chaos Expansion}
Let $(\Omega,\calF,\F,\Q)$ be a filtered probability space where
 $\F=(\calF_t)_{t\in [0,T]}$ is the natural filtration of a standard Brownian motion $W$ on $[0,T]$. As $d=1$, remark \ref{rmk:Strat} gives
 \begin{equation}\label{eq:sigW}
     \calS(W_t)= \left(1,w_t,\frac{w^2_t}{2},\ldots,\frac{w^n_t}{n!},\ldots\right).
 \end{equation}
 Hence the signature is here path-independent.
 We now recall the Wiener-Itô chaos expansion.
 \begin{thm}
Any $\calF_T-$measurable random variable $\xi$ admits the representation 
$$\xi = \E^{\Q}[\xi] + \sum_{n=1}^\infty   J_n(W_T;\phi_n), $$
where $\phi_n$ are symmetric, square integrable functions and
\begin{equation}\label{eq:chaos}
    J_n(W_T;\phi_n) &=\int_{\Delta_{n,T}} \, \phi_n\,  dw^{\otimes n}_{t} = \int_{\Delta_{n,T}} \, \phi_n(t_1,\ldots, t_n)dw_{t_1} \ldots  dw_{t_n}.
\end{equation}
Note that the above iterated integral is in the Itô sense. 
 \end{thm}
 
 \begin{remark}
 The Wiener-Itô chaos expansion is often expressed (see, e.g., \citealp{DiNunno}) as 
$$\xi = \E^{\Q}[\xi] + \sum_{n=1}^\infty n!\,  J_n(W_T;f_n), $$
where $f_n$ are again symmetric, square integrable functions. In fact, $f_n =  \frac{\phi_n}{n!}$. It is for our purposes, however, more convenient to stick to the expansion given in the previous theorem. 
 \end{remark}

 
 \begin{corollary}
 For any $\F-$adapted process $S$, there exists $(\phi_{n,t})_{n,t\,\in \N \,\times [0,T]}$ such that
 $$s_t = \E^{\Q}[s_t] + \sum_{n=1}^\infty  J_n(W_T;\phi_{n,t}), $$
 with $J_n$ as in $\eqref{eq:chaos}$.
 \end{corollary}

\begin{example}
Consider the Black-Scholes model (with zero interest rate) $$s_t= e^{\,\sigma w_t - \frac{\sigma^2}{2}t},\; t \in [0,T], \;\;\sigma>0.$$ Using the Taylor expansion of a Gaussian kernel, it can be shown that 
$$s_t = \sum_{n=0}^\infty \frac{(\sigma\sqrt{t})^n}{n!}h_n\left(\frac{w_t}{\sqrt{t}}\right),$$
where $h_n(\cdot)$ is the $n-$th (probabilist's) Hermite polynomial. Moreover, if  $$\phi_{n,t}(t_1,\ldots,t_n)= g_t^{\otimes n}(t_1,\ldots,t_n),\quad(= g_t(t_1)\cdots g_t(t_n))$$    for some $g_t\in L^2([0,T])$,  then
$$  J_n(W_T;\phi_{n,t})=   \frac{\lVert g_t\rVert^n}{n!}h_n\left(\frac{(g_t \bullet w)_t}{\lVert g_t\rVert}\right), \qquad (\lVert \cdot \rVert = \lVert \cdot \rVert_{L^2([0,T])}).$$

Hence the Wiener-Itô chaos expansion of $s_t$ is obtained using $g_t= \sigma \cdot \mathds{1}_{[0,\,t]}$. In particular for $t=T$, $(t_1,\ldots,t_n)\in \Delta_{n,T}$, we have 
$$\phi_{n,T}(t_1,\ldots,t_n)= \sigma^n\prod_{i=1}^n \mathds{1}_{[0,\,T]}(t_i)= \sigma^n.$$

On the other hand, equation $\eqref{eq:sigW}$ yields the signature decomposition
\begin{align*}
    s_T = e^{-\frac{\sigma^2}{2}T}\sum_{n=0}^\infty \frac{(\sigma \, w_T)^n}{n!}= \sum_{n=0}^\infty e^{-\frac{\sigma^2}{2}T} \sigma^n \underbrace{\frac{ w_T^n}{n!}}_{=\, J^{\circ}_n(W_T)} = 
  \langle \varphi,\calS(W_T) \rangle,
\end{align*}
with $\varphi_n= e^{-\frac{\sigma^2}{2}T}\sigma^n$. Hence the constant function $\phi_{n,T}=\sigma^n$  differs from $\varphi_n$  only by a factor $e^{-\frac{\sigma^2}{2}T}$. %Hence the simple payoff $h(W_T)$
To sum up, we have found the analogy (writing  $J_n(W_T)=J_n(W_T;\phi_n)$ if $\phi_n\equiv 1$),
\begin{align*}
    s_T = \underbrace{\sum_{n=0}^\infty e^{-\frac{\sigma^2}{2}T} \sigma^n J^{\circ}_n(W_T)}_{\text{signature decomposition}}\; = \underbrace{\sum_{n=0}^\infty \sigma^n J_n(W_T)}_{\text{Wiener-Itô chaos expansion}}.
\end{align*}

% $$\langle l_t,\calS(W_t) \rangle  = \sum_{n=0}^\infty l_{n,t}  \frac{(\sigma w_t)^n}{n!}$$
\end{example}

\begin{remark}
Consider a (possibly path-dependent) option that pays $G(W_T)$ at maturity.
If $G$ is a signature payoff, i.e. $G = \langle \varphi, \calS \rangle$ for some $\varphi\in \R^{\N}$, then  the price of the option can be expressed as (assuming zero interest rate),
$$\E^{\Q}[G(W_T)]= \langle \varphi,\E^{\Q}[\calS(W_T)] \rangle.$$
Thus the signature is an efficient option pricing tool, provided that $\E^{\Q}[\calS(W_T)]$ can be computed "easily". On the other hand, the Wiener-Itô chaos expansion does not seem to help with this regard (namely the valuation of options). Indeed, if 
$$G(W_T)= \E^{\Q}[G(W_T)] +  \sum_{n=1}^\infty   J_n(W_T;\phi_n), $$  
then taking expectation on both sides yields a trivial equality  since the iterated integrals $J_n(W_T;\phi_n)$ have zero expectation. Nevertheless, Malliavin calculus becomes of course much more relevant for hedging problems.
\end{remark}

\begin{example}
(Asian forward, Bachelier). Note that 
\begin{align*}
    \xi :&= \frac{1}{T}\int_0^T s_t dt -K\\ &= r-K +\, \frac{\sigma}{T}\int_0^T w_t dt\\
    &= \E[\xi]+\, \frac{\sigma}{T}\int_0^T (T-t) dw_t\\
    &= \E[\xi]+\, J_1(W_T;\phi_1),
\end{align*}
with $\phi_1(t)= \sigma(1-\frac{t}{T})$. Note that $\xi =r(1-T/2) -K +  \int_0^T \Delta_t ds_t$, with the hedging strategy $\Delta_t=1-\frac{t}{T}$ (linear asset liquidation).
\end{example}
%Now take $X=W$ and look for $\xi$ such that $J_n(W_T)=  n! \, \tilde{J}_n(W_T;\phi_n)$. Since $d=1$, observe that 
%$$J_n(W_T)\overset{\eqref{eq:1}}{=}\frac{w_T^n}{n!},$$
%hence $\xi= \sum_{n=0}^\infty \frac{w_T^n}{n!}= e^{\, w_T}$. %Signature solves an ODE similar to the exponential one.

==> Path_Approx/Legendre.tex <==
%\subsubsection{Connection with Legendre Polynomials}
An important property of the signature is that it uniquely characterizes a path, up to a certain equivalence relation, called tree-like equivalence (\citealp{Hambly}). In short, two paths having same signature differ at most by a \textit{tree-like path}, a specific type of loop (curve whose end points coincide). 
Hence extending a path with time$-$being strictly increasing$-$ prevents the apparition of loops and in turn ensures the injectivity of the signature map. 

This gives hope to reconstruct the (unique) path associated to a given signature. This was introduced for instance by \cite{Geng}, who came up with a geometric reconstruction using polygonal approximations for multi-dimensional Brownian paths. 
We here propose a simple algorithm, in connection with our discussion on Hilbert projections.\footnote{I thank Bruno Dupire for suggesting this interesting parallel.} %retrieve a path from some selected signature elements. 
For ease of presentation, assume $x_0=0$ and $T=1$. We start off with a useful identity.

\begin{proposition}\label{prop:100}
For the words $\alpha^{(k)} :=1\underbrace{0\ldots0}_{ k+1}\,$, $k \ge 0$, we have
\begin{equation}\label{eq:100}
    \calS_{\alpha^{(k)}}(X_{t}) = \int_0^{t} x_s \frac{(t -s)^{k}}{k!}ds,\quad \forall \, t \in [0,1]. 
\end{equation}
\end{proposition}
\begin{proof}
Fix $t\in [0,1]$. First, notice that $\calS_{\alpha^{(0)}}(X_t)=\calS_{10}(X_t) = \int_0^t x_sds$, which is $\eqref{eq:100}$. Now by induction on $k\ge 1$, uniformly on $[0,t]$,
\begin{align*}
   \calS_{\alpha^{(k)}}(X_t) = \int_0^t \calS_{\alpha^{(k-1)}}(X_u)du 
    = \int_0^t \int_0^u x_s \frac{(u -s)^{k-1}}{(k-1)!}ds\, du 
    = \int_0^t x_s\int_u^t  \frac{(u -s)^{k-1}}{(k-1)!}du\, ds
    = \int_0^t x_s \frac{(t -s)^{k}}{k!} ds.
\end{align*}
% \begin{align*}
%   \calS_{\alpha^{(k)}}(X_t) &= \int_0^t \calS_{\alpha^{(k-1)}}(X_u)du \\
%     &= \int_0^t \int_0^u x_s \frac{(u -s)^{k-1}}{(k-1)!}ds\, du \\
%     &= \int_0^t x_s\int_u^t  \frac{(u -s)^{k-1}}{(k-1)!}du\, ds\quad \text{(Fubini's theorem)}\\
%     &= \int_0^t x_s \frac{(t -s)^{k}}{k!} ds.
% \end{align*}
\end{proof}
If $\overleftarrow{X}$ denote the \textit{time reversed path}, i.e. $\overleftarrow{x_t} = x_{1-t}$, then 
$$\calS_{\alpha^{(k)}}(\overleftarrow{X_1}) = \int_0^1 \overleftarrow{x_t}\frac{(1 -t)^{k}}{k!}dt  = \int_0^1 x_t \frac{t^{k}}{k!}dt =  \frac{1}{k!}(x,m_k), $$
with the monomials $(m_k) = (t^k)$.
As mentioned in \cite{Hambly}, the signature of the time reversed path corresponds to the inverse of $\calS(X)$ in the extended tensor algebra $\calT((\R^d))= \bigoplus_{n=0}^\infty (\R^d)^{\otimes n}$. Moreover, $\calS(\overleftarrow{X_1})$ can  be  retrieved from $\calS(X_1)$ by solving a system of equations for words of increasing lengths. This goes, however,  beyond the scope of this work.  
Alternatively, we observe that
\begin{align*}
    \calS_{\alpha^{(k)}}(\overleftarrow{X_1}) %\int_0^1 x_t \frac{t^{k}}{k!}dt \\ 
    &= (-1)^{k}\int_0^1 x_t \frac{((1-t)-1)^{k}}{k!}dt \\
    &= (-1)^{k} \sum_{j=0}^k {k \choose j} \int_0^1 x_t \frac{(1-t)^{j}(-1)^{k-j}}{k!}dt \\
    %&=  \sum_{j=0}^k  \int_0^1 x_t \frac{(1-t)^{j}}{j!}dt\frac{(-1)^{-j}}{(k-j)!} \\
    &= \sum_{j=0}^{k} \calS_{\alpha^{(j)}}(X_1) \frac{(-1)^{j}}{(k-j)!}.
\end{align*}

% \begin{figure}[H]
% \caption{Shifted Legendre polynomials up to degree $3$.}
%     \centering
%     \includegraphics[scale = 0.4]{Figures/Shifted_Legendre.pdf}
    
%     \label{fig:Legendre}
% \end{figure}

\begin{figure}%[H]
    \centering
    \caption{Projected paths with $K=8\,$ basis elements. }
    \includegraphics[scale = 0.45
    ]{Figures/ProjPath.pdf}
    \label{fig:projPath}
\end{figure}
To fall within the context of orthonormal projection, we transform the monomials into the (unique) polynomial ONB of $L^2([0,1])$, constructed as follows.
Let $(p_k)$ be the Legendre polynomials (\citealp{Szego}), forming a basis of $L^2([-1,1])$. 
Then define the \textit{shifted Legendre polynomials} simply as $q_k = p_k \circ \tau_{[-1,1]}$, where 
$\tau_{[-1,1]}(t) = 2t-1, \, t\in [0,1]. $
%(Note that this is a time reparametrization!)
%The first elements are displayed in Figure \ref{fig:Legendre}. 
%The first elements reads 
The first elements write $$q_0(t) = 1, \quad q_1(t) = 2t-1, \quad q_2(t) = 6t^2 - 6t  -1.$$ 
%The family $(q_k)$ forms a orthogonal basis of $L^2([0,1])$. 
It is easily seen that the standardized polynomials $\frakF = (F_k)$,  $F_k :=  \frac{q_k}{\lVert q_k\rVert}$ form an ONB of $L^2([0,1])$. 
Next, we can write $F_k(t)= \sum\limits_{j\le k} a_{kj}t^j$, with coefficients $a_{kj}$ obtained for instance from \textit{Rodrigues' formula} (\citealp[Section 4.3]{Szego}). As usual,  $X^{K,\frakF} = \sum\limits_{k\le K} \xi_k F_k$, where the Fourier coefficients become
$$\xi_k = (X,F_k) = \sum_{j\le k} a_{kj}\, (X,m_j) = \sum_{j \le k} b_{k,j}\, \calS_{\alpha^{(j)}}(\overleftarrow{X_1}), \quad b_{k,j} = j!\, a_{k,j}.$$
Therefore,  having signature elements up to order $K \ge 1$ yields
\begin{align*}
    x^{K,\frakF}_t 
    = \sum_{k\le K} \xi_k F_k(t)
    %= \sum_{k \le K} \sum_{j\le k} b_{k,j}\, \calS_{\alpha^{(j)}}(\overleftarrow{X_1}) F_k(t)
    = \sum_{j \le K} \calS_{\alpha^{(j)}}(\overleftarrow{X_1})  G_j(t),  \qquad G_j(t) = \sum\limits_{k\le j \le K} b_{k,j}\,  F_k(t).
\end{align*}
Altogether, we have seen that the signature elements $(\calS_{\alpha^{(j)}})$ generate the $L^2$ products of the path with the monomials$-$and in turn, with the Legendre polynomials$-$from which a projection of the path is available.
The reconstruction algorithm is  summarized below. %Taking $K$ too large (say, larger than $15$) may introduce exploding oscillations. 
\vspace{3mm}
\begin{mybox}{black}{\textbf{Path Reconstruction Algorithm}}
%\begin{tcolorbox}
\begin{enumerate}
\setlength \itemsep{1ex}
\item \textbf{Input:} (i) Signature elements $\calS_{\alpha^{(j)}}(X_1)$, $\; 0\le j \le K$.

      \hspace{9mm}  (ii) Time grid $0 = t_0 < \ldots < t_N =1$.
    
    \item \textbf{Offline:} For $0 \le j \le K, \,\;  0\le n \le N$,  calculate $G_j(t_n)$. 
    \item \textbf{Online}: For $0\le j \le K$,  compute  $\calS_{\alpha^{(j)}}(\overleftarrow{X_1})$.
    \item \textbf{Output}: For $0\le n \le N$, return $x^{K,\frakF}_{t_n} = \sum_{j\le K} \calS_{\alpha^{(j)}}(\overleftarrow{X_1}) G_j(t_n)$.
\end{enumerate}

%\end{tcolorbox}
\end{mybox}



==> Path_Approx/ProjTruncSig.tex <==

\newpage
\subsection{$L^2(\Q \otimes dt)$ projection using truncated signature.}

Given $(\calS_{\alpha})_{|\alpha|_0\,  \le \, K}$, solve

$$\min_{\frakF } \left \lVert X^{K,\frakF} - X \right \rVert_{L^2(\Q \otimes dt)}, \quad x^{K,\frakF}_t = \sum_{|\alpha|_0\,  \le \, K} \calS_{\alpha} F_\alpha(t),$$
for a family of deterministic functions $\frakF = (F_{\alpha})$.
\begin{example}
(Legendre Polynomials) Set $F_{\alpha^{(j)}} = G_j$ (see previous part) and $F_{\alpha} = 0$ otherwise.
\end{example}

\subsection{Nonlinear combination}
Take $T =1$, $x_0 = 0$ $\Q-$a.s. and $K=3$. Relevant quantities up to order $3$ (see figure on next page) are 

\begin{itemize}
\item \textbf{Order $0$}: $\calS_{\emptyset} = 1$.  (\textbf{Constant})
    \item \textbf{Order $1$}: $\calS_{(1)} = x_1 =: x$.  (\textbf{Terminal value})
    \item \textbf{Order $2$}: $\calS_{(1,0)} = \int_0^1 x_t dt  =: \bar{x}$.  (\textbf{Average})
    \item \textbf{Order $3$}: $ \int_0^1 (x_t - \bar{x})^2 dt  =: \bar{\bar{x}}$.  (\textbf{Variation}), $ \int_0^1 (x_t - \bar{x}) t dt  =: \underbar{\bar{x}}$  (\textbf{Chronology}). 
\end{itemize}
Note that $\bar{\bar{x}}$ and $\underbar{\bar{x}}$ are functions of signature elements up to order $3$, since 
\begin{align*}
\bar{\bar{x}} &= \int_0^1 x_t^2 dt - \bar{x}^2 = 2 \calS_{(1,1,0)} - \bb{\calS_{(1,0)}^2}, \\
\underbar{\bar{x}} &=  \underbrace{\calS_{(1,0)} -\calS_{(1,0,0)}}_{= \, \int_0^1 x_t\, t dt }  - \underbrace{\frac{1}{2}\calS_{(1,0)}}_{= \, \int_0^1 \bar{x}\, t dt } = \frac{1}{2}\calS_{(1,0)} - \calS_{(1,0,0)}.
\end{align*}
Now look at a  nonlinear combination, i.e. 
$$ x^{K,\frakF}_t = \sum_{|\alpha|_0\,  \le \, K}  g_{\alpha}(\calS_{\alpha}) F_\alpha(t)$$
(e.g. take \bb{$g_{(1,0)}(s) = s^2$  for $\bar{\bar{x}}$}), such that

$$\{\alpha \, | \, F_{\alpha} \ne 0\} \subseteq \{\emptyset, (1), (1,0), (1,1,0), (1,0,0)\}.$$

\newpage

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.3]{Figures/Path_Construction_Sig.jpg}
\end{figure}

\newpage

==> TerminalFunctional/PBSDE.tex <==
\subsection{PBSDEs (?)}
This seems closely related to (F)BSDEs: if $Y=f(X)$, then 
$$y_t = y_T - \int_t^T \varphi(s, Y_s, Z_s)ds -  \int_t^T z_s \circ dx_s, $$
with $z_t = \Delta_x f(X_t)$, $\varphi(t,X_t) = \Delta_t f(X_t)$, or if 
$$dx_t = \mu(X_t)dt + \sigma(X_t) \circ dw_t, $$
then
$$y_t = y_T - \int_t^T \varphi(s,Y_s,Z_s)ds -  \int_t^T z_s \circ dw_s, $$
with $z_t = \sigma(X_s) \Delta_x f(X_t) $,\,  $\varphi(t,X_t,Z_t) = \frac{\mu(X_t)}{\sigma(X_t)} z_t + \Delta_t f(X_t)$ if $0 \notin \sigma(\Lambda) $  \textbf{(FBSDE)}.

\bb{See Peng and Wang}


==> TerminalFunctional/TermFunc.tex <==

\textbf{Given}: Terminal functional $g:\Lambda_T \to \R$. Note that the time derivatives for $g$ cannot be defined, but the space derivative can. 
\\
\textbf{Goal}: Find a functional $f$ such that
\begin{itemize}
    \item $f\in \C^K$ for some $K$ (smoothness)
    \item $f(X_T) = g(X_T) $
\end{itemize}
The set $\Gamma^K_g = \Gamma_g \, \cap \, \C^K$, $\Gamma_g = \{f:\Lambda \to \R \, |\, g(X_T) = f(X_T) \}$ is in general not a singleton. Hence we need an additional criterion for $f$.  For instance, solve an optimization program,
$$\min_{f \in \Gamma^K_g} \; l( f),$$
for some loss function $l: \Gamma^K_{g} \to \R$. 
\subsection{Losses}
\subsubsection{$L^2$ projection }
Define for $t\in [0,T]$
$$ l_t(f) = \lVert f(X_t) - g(X_T) \rVert_{L^2(\Q)}^2, $$
which gives the conditioned expectation $f(X_t) = \E^{\Q}[g(X_T) \, |\, X_t]$, i.e. the price of an option with (path-dependent) payoff $g$. We indeed have $f(X_t) \overset{t\uparrow T}{\longrightarrow} g(X_T)$. Then $f$ also minimizes the total distance
$$l(f) = \int_0^T l_t(f)dt = \lVert f(X) - g(X_T) \rVert_{L^2(\Q\, \otimes \,dt)}^2. $$
Why penalizing large deviations from $g(X_T)$ if the terminal constraint is already here?

\subsubsection{Time Variation}
$$l(f) = \E^{\Q}[(\calV f)(X_T)],$$
with the (pathwise) time variation
$$(\calV f)(X_T) = \int_0^T (f(X_t) - \bar{f})^2 dt, \quad \bar{f} = \frac{1}{T} \int_0^T f(X_t)dt. $$

\subsection{Intrinsic Functional}
\begin{definition}
    The intrinsic functional associated to $g:\Lambda_T \to \R$ is defined as $$\iota(X_t) := g(X_{t,T-t}),\quad t\in [0,T].$$
\end{definition}

\bb{Use an operator: $\calI: \R^{\Lambda_T} \to \R^{\Lambda}$, $\calI g =f $.}

Derivatives of $\iota\,$:
\begin{align*}
    \Delta_x \iota(X_t) &= \lim_{h \to 0} \frac{ \iota(X^h_t)- \iota(X_t)}{h}
    = \lim_{h \to 0} \frac{g((X^h)_{t,T-t})- g(X_{t,T-t})}{h}, \quad \text{(bump at $t$)}\\\\
    \Delta_t \iota(X_t) &= \lim_{\delta t \downarrow 0} \frac{ \iota(X_{t,\delta t})- \iota(X_t)}{h}
    = \lim_{\delta t \downarrow 0} \frac{g(X_{t,\delta t + (T-t - \delta t)})- g(X_{t,T-t})}{\delta t} = 0.
\end{align*}
The space derivative of $\iota$ is somewhat similar the Malliavin derivative of $g$, as the whole future path is shocked at time $t$.

\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.2]{Figures/IntrinsicFuncDerivative.jpg}
\end{figure}
Now decompose any $f\in \Gamma_g^K$ as
$$f = \iota + h, \quad h\in \Gamma_{\boldsymbol{0}}.$$
When is it optimal to choose $h \equiv 0$?

\begin{example}
Let $g(X_T)=\frac{1}{T}\int_0^T x_s ds$ and $f(X_t) = \frac{1}{t}\int_0^t x_s ds$. The intrinsic functional is 
$$\iota(X_t)  =\frac{1}{T}\int_0^T x_{s\wedge t} ds  = \lambda_t \underbrace{\frac{1}{t}\int_0^t x_s ds}_{\text{average over $[0,t]$}} + (1-\lambda_t)\underbrace{x_t}_{\mathclap{\text{average over $[t,T]$}}}\,, \quad \lambda_t = \frac{t}{T}.$$
 Therefore, 
$$f(X_t) = \iota(X_t) + \frac{T-t}{t}(\iota(X_t)-x_t) = \iota(X_t) +  h(X_t), $$
with $h(X_t) = \left(\frac{1}{t} - \frac{1}{T}\right) \int_0^t (x_s-x_t) ds \overset{t\uparrow T}{\longrightarrow} 0$.

\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.2]{Figures/IntrinsicFuncAsian.jpg}
\end{figure}

\end{example}

\begin{example}
Let $g(X_T)=x^2_T$ and consider its Bachelier price with volatility $\sigma$, i.e. 
$$f_{\sigma}(X_t) = \E^{\Q_{\sigma}}[ x_T^2\, | \, X_t] = \underbrace{x_t^2}_{= \, \iota(X_t)} + \underbrace{\sigma^2(T-t)}_{=\,h_{\sigma}(X_t)}.$$
Hence $f_{\sigma} \overset{\sigma \downarrow 0}{\longrightarrow} \iota$. 
% If $X$ is seen as the log price, then 
% $$f_{\sigma}(X_t) = \quad \lambda_t \underbrace{\frac{T}{t} x_t^2}_{\mathclap{\text{Annualized historical variance}}}\quad  +\quad  (1-\lambda_t) \underbrace{\sigma^2 T}_{\mathclap{\text{Total variance}}} $$
\end{example}

\begin{example}
Let $g(X_T)=\langle X \rangle_T$, $X$ L\'evy process and $f$ is the conditioned expectation. This gives, 
$$f(X_t) = \E^{\Q}[ \langle X \rangle_T\, | \, X_t] = \underbrace{\langle X \rangle_t}_{= \, \iota(X_t)} + \underbrace{\E^{\Q}[\langle X \rangle_{T-t}]}_{=\,h(X_t)}.$$
\end{example}

The time variation reads 
$$\calV f = \calV \iota + \calV h + 2\, (\iota - \bar{\iota},h - \bar{h})_{L^2([0,T])}.$$

% \subsection{Optimality among the extended paths}
% Fix $t <T$ and restrict to the family of functionals
% $$f_Z(X_t) = g(X_t \oplus Z_{T-t}),\quad (X_t \oplus Z_{T-t})(s) = x_{s \wedge t} + Z_{T-t}((s-t) \vee 0)$$
% where $Z_{T-t} \in \Lambda_{T-t} $ is $\sigma(X_t)-$measurable with $Z_{T-t}(0) = 0$. When $Z_{T-t} \equiv 0$, we fall back on the intrinsic functional. 

% \begin{example}
% Take again $g(X_T)=x^2_T$ and choose $Z_{T-t}(s)=  \sigma \frac{s-t}{\sqrt{T-t}} $, $s\in [t,T]$. Then 
% $$f_{Z}(X_t) = (x_t + \sigma \sqrt{T-t})^2 = \E^{\Q_{\sigma}}[ x_T^2\, | \, X_t] + 2x_t \, \sigma \, \sqrt{T-t}.$$
% % If $X$ is seen as the log price, then 
% % $$f_{\sigma}(X_t) = \quad \lambda_t \underbrace{\frac{T}{t} x_t^2}_{\mathclap{\text{Annualized historical variance}}}\quad  +\quad  (1-\lambda_t) \underbrace{\sigma^2 T}_{\mathclap{\text{Total variance}}} $$
% \end{example}

\subsection{Applications}
\begin{itemize}
    \item Hedging: $f(X_t) = \int_0^t \varphi(X_s) dx_s$?
    \item American option: Requires $g$ to be defined on $\Lambda$, in which case we simply take the intrinsic value $g(X_t)$. Replace the cont. value by $$\E^{\Q} [g(X_{t,\tau-t})] = \int_t^T g(X_{t,s-t}) \Q(\tau \in ds)?$$
\end{itemize}

==> TerminalFunctional/TermFuncMain.tex <==
\newpage
\section{\blue{Terminal functional and Path-Dependent BSDEs (PBSDE) (relevant?)}}
 
 \input{TerminalFunctional/TermFunc}
 
 \input{TerminalFunctional/PBSDE}
